Large Language Models are Learnable Planners for Long-Term Recommendation

Planning for both immediate and long-term benefits becomes increasingly important in recommendation. Existing methods apply Reinforcement Learning (RL) to learn planning capacity by maximizing cumulative reward for long-term recommendation. However, the scarcity of recommendation data presents challenges such as instability and susceptibility to overfitting when training RL models from scratch, resulting in sub-optimal performance. In this light, we propose to leverage the remarkable planning capabilities over sparse data of Large Language Models (LLMs) for long-term recommendation. The key to achieving the target lies in formulating a guidance plan following principles of enhancing long-term engagement and grounding the plan to effective and executable actions in a personalized manner. To this end, we propose a Bi-level Learnable LLM Planner framework, which consists of a set of LLM instances and breaks down the learning process into macro-learning and micro-learning to learn macro-level guidance and micro-level personalized recommendation policies, respectively. Extensive experiments validate that the framework facilitates the planning ability of LLMs for long-term recommendation. Our code and data can be found at https://github.com/jizhi-zhang/BiLLP.

==> backup/1-Introduction.tex <==
% Recommendation systems have gained widespread adoption in contemporary society to alleviate the overwhelming burden of information overload \cite{DBLP:journals/corr/abs-2010-03240}. 
% % Traditionally, researchers primarily focused on the static recommendation setting \cite{DBLP:conf/sigir/0001DWLZ020, DBLP:conf/icdm/KangM18}, which digs up users' static interests from historical data and subsequently provides recommendations tailored to their preferences. 
% Traditionally, researchers primarily focused on immediate responses such as clicks and likes.
% However, such a greedy recommendation strategy tends to excessively cater to users' immediate interests, neglecting the importance of planning for long-term engagement \cite{DBLP:conf/kdd/WangSXBSRCCC22}. This will result in the user becoming confined within an echo chamber of preferred information and items, which is also called ``filter bubbles''. The homogenization of recommendations derived from filter bubbles may make users bored and jeopardize their long-term engagement.
%%% wentao 

Recommendation systems have gained widespread adoption in contemporary society to alleviate the overwhelming burden of information overload~\cite{DBLP:journals/corr/abs-2010-03240}. 
Traditionally, researchers primarily focused on optimizing users' immediate responses (typically clicks) to maximize instant benefits~\cite{wu2017returning}.
However, such a greedy recommendation strategy tends to cater to users' immediate interests excessively, neglecting the importance of planning for long-term engagement \cite{DBLP:conf/kdd/WangSXBSRCCC22}. This will result in the user becoming confined within an echo chamber of preferred information and items, which is also called ``filter bubbles''. The homogenization of recommendations derived from filter bubbles may make users bored and jeopardize their long-term engagement.

%which persistent consumption gradually exhausts the drive to engage. 
% Homogenizing recommendations derived from filter bubbles would gradually exhaust users' drive to engage, jeopardizing their long-term engagement.
%Persistent and homogeneous recommendations would gradually exhaust users' drive to engage, jeopardize their long-term engagement.



% 方法总结：2类： 总结方法特点（偏向于idea的总结）（early approach 放related work)  开头强调planning   RL planning   why not planning 的不好

% RL 不擅长长尾item的推荐
% RL 收敛慢
% To maximize users' long-term engagement, it is crucial to incorporate planning capabilities to mitigate the effects of filter bubbles, where the recommendation decisions should consider not only immediate benefits but also long-term ramifications. Traditionally, researchers employ the planning capability of Reinforcement Learning (RL) algorithms to optimize long-term user satisfaction \cite{DBLP:journals/csur/AfsarCF23, DBLP:conf/www/00010WZXYZJG23, DBLP:conf/www/0001XZX0ZWZXZJG23}, with RL's planning capacity stemming from its training process aimed at maximizing cumulative reward.
% Despite RL's inherent capacity, the scarcity of recommendation data presents challenges such as instability and susceptibility to overfitting when training RL models from scratch. Consequently, RL-based recommendation models often exhibit limited planning ability on long-tail items and result in subpar performance. Moreover, learning RL policies requires a large amount of interaction data, rendering their implementation in online recommender systems impracticable.
% Therefore, finding an effective planner that can learn robustly and efficiently on sparse data to address filter bubbles becomes critical to maximize users' long-term engagement.
%%% wentao 

To maximize users' long-term engagement, it is crucial to incorporate planning capabilities to mitigate the effects of filter bubbles, where the recommendation decisions should consider not only immediate benefits but also long-term ramifications. Traditionally, researchers employ the planning capability of Reinforcement Learning (RL) algorithms to optimize long-term user satisfaction \cite{DBLP:journals/csur/AfsarCF23, DBLP:conf/www/00010WZXYZJG23, DBLP:conf/www/0001XZX0ZWZXZJG23}, with RL's planning capacity stemming from its training process aimed at maximizing cumulative reward.
Despite RL's inherent capacity, the scarcity of recommendation data presents challenges such as instability and susceptibility to overfitting when training RL models from scratch. Consequently, RL-based recommendation models often exhibit limited planning ability on long-tail items and result in subpar performance. 
% 收敛慢。。换一个理由
Moreover, learning RL policies requires a large amount of interaction data, rendering their implementation in online recommender systems impracticable.
Therefore, finding an effective planner that can learn robustly and efficiently on sparse data to address filter bubbles becomes critical to maximize users' long-term engagement.


% 开始powerful extern knowledge
% 增加为什么LLM能够在稀疏任务上表现好
Recently, Large Language Models (LLMs) have emerged with powerful planning capabilities for solving complex tasks \cite{DBLP:conf/iclr/YaoZYDSN023, shinn2023reflexion}, which are capable of breaking down complex tasks into subtasks and then executing them sequentially. Multiple rounds of recommendation can be considered as complex tasks, where LLMs allow for the strategic arrangement of item recommendations to the user, thereby facilitating users' long-term engagement. 
The extensive world knowledge possessed by LLMs resulting from pre-training confers them with robust planning capabilities despite sparse recommendation data. The planning policy caters to individual user preferences while having appropriate diversity to alleviate the filter bubble problem.
% The powerful planning ability of LLM stems from its massive world knowledge from pre-training, which enables personalized interaction sequences that cater to individual user preferences while having appropriate diversity to alleviate the filter bubble problem. 

% 分两段，challenge he method
%  控制cost  解决gap

While LLMs hold significant promise as planners, due to the substantial divergence between the pre-training scenario and the recommendation scenario, the direct application of LLMs in the interactive recommendation faces compatibility issues and often results in subpar performance. Fine-tuning LLM on recommendation data provides a direct approach to bridging the gap. However, this process comes with substantial computational costs and is not applicable to closed-source models, like GPT-4. 
% Wentao version



% While LLMs hold significant promise as planners, due to the substantial divergence between the pre-training scenario and the recommendation scenario, the direct application of LLMs in the interactive recommendation faces compatibility issues and often results in subpar performance. We need to stimulate the planning capabilities of LLMs specifically for recommendation tasks.  This is a non-trivial task. The planning required for recommendations is highly complex: it involves reasoning distinct strategies for different users, and the planning needs to be fine-grained down to each individual item.

%在这项工作中，我们探讨了利用LLMs的规划能力进行长期参与推荐的核心主题。鉴于微调方法的巨大成本，我们考虑发扬LLM in-context learning的能力，直接从包含先验成功及失败的language feedback去学习如何更好地规划。但是，这里所需要的planning能力是非常复杂的，一方面plan被需要保证span long time horizons，另一方面，plan是需要非常个性化地且具体到具体的item推荐策略。如何令大模型高效地学会这样planning能力是关键挑战。 
% In this work, we explore the central theme of harnessing the planning abilities of LLMs for long-term engagement in recommendations. Considering the significant cost of fine-tuning methods, we contemplate leveraging the in-context learning capability of LLMs, directly learning how to plan better from language feedback. The language feedback includes prior successes and failures, which could serve as "semantic gradients", providing a concrete direction for LLM to improve upon~\cite{shinn2023reflexion}. However, the required planning abilities are highly intricate, and direct learning is non-trivial. On the one hand, the planning must ensure coverage over long time horizons. On the other hand, the planning must be highly personalized and specific to individual item recommendation strategies from a vast and diverse space of items. 

% In this work, we explore the central theme of harnessing the planning capabilities of LLMs for fostering long-term engagement in recommendations. The key is to specify the planning abilities for the recommendation. Given the substantial cost associated with fine-tuning methods, we consider achieving the goal by learning from language feedback with in-context learning. The language feedback, encompassing both prior successes and failures, could serve as "semantic gradients," providing a tangible direction for LLM to improve upon. However, direct learning is non-trivial, since the requisite planning abilities are highly intricate. On one hand, the desired planning coverage over a long time horizon. On the other hand, planning must be highly personalized and specific to individual item recommendation strategies within a vast and diverse space of items. 

% In this study, we explore the central theme of harnessing the planning capabilities of LLMs to optimize long-term engagement in recommendations. The key lies in tailoring the planning capabilities of LLMs to align with the recommendation. We contemplate achieving this alignment through learning from language feedback via in-context learning, given the substantial cost associated with fine-tuning methods. The language feedback, encapsulating both prior successes and failures, can act as "semantic gradients," providing tangible directions for LLMs to improve upon. However, direct learning the desired planning is non-trivial, given the highly complex nature of the required planning abilities. On one hand, the planning naturally spans a long time horizon towards optimizing the long-term engagement goal. On the other hand, it must be highly personalized and specific to individual item recommendation strategies within a vast and diverse space of items.


% We need to inspire the LLMs' planning abilities for recommendation, which is non-trivial. The planning required for recommendations is more intricate: this ability needs to be personalized and needs to be very fine-grained to the item space for each decision.  
%To stimulate planning capabilities in recommendations, specific and carefully designed strategies are needed. However, this is non-trivial. 
% The planning required for recommendations is more intricate compared to other tasks: it involves long-term considerations, and on the other hand, this ability needs to be personalized, with each decision finely tuned to specific items. Attempting to instill such capabilities in a "one-step" manner poses a significant challenge.

%Fine-tuning LLM on recommendation data provides a direct approach to bridging the gap. However, this process comes with substantial computational costs and is not applicable to closed-source models, like GPT-4. 


To bridge the gap, in this work, we introduce \textbf{RecPlanner}, a bi-level learnable LLM planner framework for the interactive recommendation that learns from language feedback without fine-tuning. As shown in Figure~\ref{fig:main_structure}, it consists of bi-level learning mechanisms: macro-learning, which involves the rapid acquisition of macro-level recommendation planning guidance, and micro-learning, which focuses on learning personalized planning policies. By integrating the two learning mechanisms, we efficiently adopt the pre-trained LLMs to personalized recommendation planners without fine-tuning. All the learning processes are implemented by updating the equipped text memory in each module. To further enhance the learning speed and effectiveness of micro-learning, drawing an analogy to the A2C algorithm~\cite{}, we propose a novel \textit{Critic Module} that serves to augment the updating process of the Actor policy. The \textit{Critic Module} evaluates the quality of various actions in the current state, thereby assisting the Actor policy in making immediate updates while mitigating the issue of high variance estimations of Q-values.
% % By interacting with the equipped memory component in each module, LLMs could quickly adapt to recommendation tasks without fine-tuning. 
% %We incorporate two In-Context Learning strategies: the Macro-learning strategy and the Micro-learning strategy, which learn high-level guidance and low-level action suggestions respectively.


% To this end, we introduce \textbf{RecPlanner}, a bi-level learnable LLM planner framework for the interactive recommendation that learns from language feedback without fine-tuning. As shown in Figure~\ref{fig:main_structure}, it consists of bi-level learning mechanisms: macro-learning, which involves the rapid acquisition of macro-level recommendation planning guidance, and micro-learning, which focuses on learning personalized planning policies. By integrating the two learning mechanisms, we efficiently adopt the pre-trained LLMs to personalized recommendation planners without fine-tuning. All the learning processes are implemented by updating the equipped text memory in each module. To further enhance the learning speed and effectiveness of micro-learning, drawing an analogy to the A2C algorithm~\cite{}, we propose a novel \textit{Critic Module} that serves to augment the updating process of the Actor policy. The \textit{Critic Module} evaluates the quality of various actions in the current state, thereby assisting the Actor policy in making immediate updates while mitigating the issue of high variance estimations of Q-values.


% To address this, we introduce \textbf{RecPlanner}, a bi-level learnable LLM planning framework designed for interactive recommendations. It learns directly from language feedback without the need for fine-tuning. To simplify the learning process, it employs a hierarchical mechanism, breaking the learning down into macro-learning, which acquires high-level and coarse-grained policy at the semantic level (e.g., "xxxx"), and micro-learning, which refines personalized policy based on the macro-level result and user characteristics. These mechanisms are implemented by the Planner-Reflector and Actor-Critic, respectively. The Planner and Actor are large model instances equipped with memory modules, offering policies for the two hierarchical levels. The Reflector and Critic are evaluation modules based on LLM, offering rapid feedback or assessments on long-term objectives for the Planner and Actor, thereby helping enhance their policies.

%  xxx memory 
% 先将框架
% 后讲xxx
%  实验结果验证
\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{Figure/main_structure.pdf}
  \caption{The overview of the proposed XXX architecture, which contains four major modules: Reflector, Planner, Actor, and Critic. The black line indicates that the data is used as a prompt input to the next module, and the red line indicates that the data is used to update the memory of the next module.}
  \label{fig:main_structure}
\end{figure*}

The main contributions of the paper can be summarized as follows:
\begin{itemize}[leftmargin=*]
    \item To our best knowledge, we are the first to apply the planning ability of LLMs to alleviate the filter bubbles problems and thus maximize users' long-term engagement.
    % 可解释加入到框架特点中
    \item We propose \textbf{RecPlanner}, a bi-level learnable LLM planner framework to improve the planning ability of LLMs in the interactive recommendation system.
    \item Drawing an analogy to the A2C algorithm, we propose the \textit{Critic Module} to augment the updating process of the Actor policy, mitigating the issue of high variance estimations of Q-values
    \item Extensive experimental findings provide empirical evidence supporting the capability of LLMs to effectively plan the sequence of items in interactive recommendation scenarios. 
    %These experiments demonstrate that LLMs possess not only strong planning ability but also notable interpretability and generalization.
\end{itemize}





==> backup/1_intro.tex <==
Recommendation systems have gained widespread adoption in contemporary society to alleviate the overwhelming burden of information overload \cite{DBLP:journals/corr/abs-2010-03240}. Traditionally, researchers primarily focused on the static recommendation setting \cite{DBLP:conf/sigir/0001DWLZ020, DBLP:conf/icdm/KangM18}, which digs up users' static interests from historical data and subsequently provides recommendations tailored to their preferences. However, such a greedy recommendation strategy tends to excessively cater to users' immediate interests, neglecting the importance of planning for long-term engagement \cite{DBLP:conf/kdd/WangSXBSRCCC22}. This will result in the user becoming confined within an echo chamber of preferred information and items, which is also called ``filter bubbles''. The homogenization of recommendations derived from filter bubbles may make users bored and jeopardize their long-term engagement.

%To maximize users' long-term engagement, it is imperative to move beyond the Next Item Prediction framework and instead adopt a interactive recommendation system that treats recommendations as a decision-making process aimed at maximizing long-term user satisfaction.

% 方法总结：2类： 总结方法特点（偏向于idea的总结）（early approach 放related work)  开头强调planning   RL planning   why not planning 的不好

% RL 不擅长长尾item的推荐
% RL 收敛慢
To maximize users' long-term engagement, it is crucial to incorporate planning capabilities to mitigate the effects of filter bubbles, where the recommendation decisions should consider not only immediate benefits but also long-term ramifications. Traditionally, researchers employ the planning capability of Reinforcement Learning (RL) algorithms to optimize long-term user satisfaction \cite{DBLP:journals/csur/AfsarCF23, DBLP:conf/www/00010WZXYZJG23, DBLP:conf/www/0001XZX0ZWZXZJG23}, with RL's planning capacity stemming from its training process aimed at maximizing cumulative reward.
Despite RL's inherent capacity, the scarcity of recommendation data presents challenges such as instability and susceptibility to overfitting when training RL models from scratch. Consequently, RL-based recommendation models often exhibit limited planning ability on long-tail items and result in subpar performance. Moreover, learning RL policies requires a large amount of interaction data, rendering their implementation in online recommender systems impracticable.
Therefore, finding an effective planner that can learn robustly and efficiently on sparse data to address filter bubbles becomes critical to maximize users' long-term engagement.



% 增加为什么LLM能够在稀疏任务上表现好
Recently, Large Language Models (LLMs) have emerged with powerful planning capabilities for solving complex tasks \cite{DBLP:conf/iclr/YaoZYDSN023, shinn2023reflexion}, which are capable of breaking down complex tasks into subtasks and then executing them sequentially. Multiple rounds of recommendation can be considered as complex tasks, where LLMs allow for the strategic arrangement of item recommendations to the user, thereby facilitating users' long-term engagement. 
The extensive world knowledge possessed by LLMs resulting from pre-training confers them with robust planning capabilities despite sparse recommendation data. The planning policy caters to individual user preferences while having appropriate diversity to alleviate the filter bubble problem.
% The powerful planning ability of LLM stems from its massive world knowledge from pre-training, which enables personalized interaction sequences that cater to individual user preferences while having appropriate diversity to alleviate the filter bubble problem. 

% 分两段，challenge he method
%  控制cost  解决gap

While LLMs hold significant promise as planners, due to the substantial divergence between the pre-training scenario and the recommendation scenario, the direct application of LLMs in the interactive recommendation faces compatibility issues and often results in subpar performance. Fine-tuning LLM on recommendation data provides a direct approach to bridging the gap. However, this process comes with substantial computational costs and is not applicable to closed-source models, like GPT-4. 

To bridge the gap, in this work, we introduce \textbf{RecPlanner}, a bi-level learnable LLM planner framework for the interactive recommendation that learns from language feedback without fine-tuning. As shown in Figure~\ref{fig:main_structure}, it consists of bi-level learning mechanisms: macro-learning, which involves the rapid acquisition of macro-level recommendation planning guidance, and micro-learning, which focuses on learning personalized planning policies. By integrating the two learning mechanisms, we efficiently adopt the pre-trained LLMs to personalized recommendation planners without fine-tuning. All the learning processes are implemented by updating the equipped text memory in each module. To further enhance the learning speed and effectiveness of micro-learning, drawing an analogy to the A2C algorithm~\cite{}, we propose a novel \textit{Critic Module} that serves to augment the updating process of the Actor policy. The \textit{Critic Module} evaluates the quality of various actions in the current state, thereby assisting the Actor policy in making immediate updates while mitigating the issue of high variance estimations of Q-values.
% By interacting with the equipped memory component in each module, LLMs could quickly adapt to recommendation tasks without fine-tuning. 
%We incorporate two In-Context Learning strategies: the Macro-learning strategy and the Micro-learning strategy, which learn high-level guidance and low-level action suggestions respectively.

%  xxx memory 
% 先将框架
% 后讲xxx
%  实验结果验证
\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{Figure/main_structure.pdf}
  \caption{The overview of the proposed XXX architecture, which contains four major modules: Reflector, Planner, Actor, and Critic. The black line indicates that the data is used as a prompt input to the next module, and the red line indicates that the data is used to update the memory of the next module.}
  \label{fig:main_structure}
\end{figure*}

The main contributions of the paper can be summarized as follows:
\begin{itemize}[leftmargin=*]
    \item To our best knowledge, we are the first to apply the planning ability of LLMs to the interactive recommendation to alleviate the filter bubbles problems.
    % 可解释加入到框架特点中
    \item We propose \textbf{RecPlanner}, a bi-level learnable LLM planner framework to improve the planning ability of LLMs in the interactive recommendation system.
    \item Drawing an analogy to the A2C algorithm, we propose the \textit{Critic Module} to augment the updating process of the Actor policy, mitigating the issue of high variance estimations of Q-values
    \item Extensive experimental findings provide empirical evidence supporting the capability of LLMs to effectively plan the sequence of items in interactive recommendation scenarios. 
    %These experiments demonstrate that LLMs possess not only strong planning ability but also notable interpretability and generalization.
\end{itemize}




